Hierarchies of Inefficient Kernelizability

The framework of Bodlaender et al. (ICALP 2008) and Fortnow and Santhanam (STOC 2008) allows us to exclude the existence of polynomial kernels for a range of problems under reasonable complexity-theoretical assumptions. However, there are also some issues that are not addressed by this framework, including the existence of Turing kernels such as the "kernelization" of Leaf Out Branching(k) into a disjunction over n instances of size poly(k). Observing that Turing kernels are preserved by polynomial parametric transformations, we define a kernelization hardness hierarchy, akin to the M- and W-hierarchy of ordinary parameterized complexity, by the PPT-closure of problems that seem likely to be fundamentally hard for efficient Turing kernelization. We find that several previously considered problems are complete for our fundamental hardness class, including Min Ones d-SAT(k), Binary NDTM Halting(k), Connected Vertex Cover(k), and Clique(k log n), the clique problem parameterized by k log n.

==> abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Abstract
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The framework of Bodlaender et al.~(ICALP 2008) and Fortnow and
Santhanam~(STOC 2008) allows us to exclude the existence of
polynomial kernels for a range of problems under reasonable
complexity-theoretical assumptions. However, there are also
some issues that are not addressed by this framework, including
the existence of Turing kernels such as the ``kernelization''
of \textsc{Leaf Out Branching$(k)$} into a disjunction over~$n$
instances of size poly$(k)$.

\hspace{10pt} Observing that Turing kernels are preserved by
polynomial parametric transformations, we define a
\emph{kernelization hardness} hierarchy, akin to the M- and
W-hierarchy of ordinary parameterized complexity, by the
PPT-closure of problems that seem likely to be fundamentally
hard for efficient Turing kernelization. We find that several
previously considered problems are complete for our fundamental
hardness class, including \textsc{Min Ones~$d$-SAT$(k)$},
\textsc{Binary NDTM Halting$(k)$}, \textsc{Connected Vertex
Cover$(k)$}, and \textsc{Clique$(k \log n)$}, the clique
problem parameterized by~$k \log n$.


==> section6.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Section: Discussion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We have defined a hierarchy of classes of inefficient
kernelization, akin to the M- and W-hierarchy of parameterized
intractability. The fundamental distinction in the new
hierarchy is between problems admitting polynomial Turing
kernels (Turing-\PK) and \WK[1]-hard problems. This distinction
does not seem to be addressable by previous lower-bound
frameworks, as evidenced by problems such as \textsc{Leaf Out
Branching}$(k)$ and \textsc{Clique}$(\Delta)$, which admit
polynomial Turing kernels but no standard polynomial kernels
unless the polynomial hierarchy collapses. Thus, \WK[1] $\not
\subseteq$ Turing-\PK\ is a new conjecture in kernelization
theory. We showed that many natural parameterized problems to
which the kernelization lower bounds apply are \WK[1]-complete,
indicating that the class is natural. Of course, our examples provide only a partial image of the \WK[1] landscape. For example, the various kernelizability dichotomies that have
been shown for CSP problems~\cite{KratschWahlstrom2010,KratschMarxWahlstrom2010}
can be shown to imply dichotomies between problems with
polynomial kernels and \WK[1]-complete problems (and
in some cases the third class of W[1]-hard problems).


Still, several questions remain. One is the \WK[1]-hardness of
\textsc{Path$(k)$} and \textsc{Cycle$(k)$}; for these problems,
we have only lower bound proofs in the framework of Bodlaender
\emph{et al.}~\cite{Bodlaender-et-al2009a}, leaving the
question of Turing kernels open. There are also several
problems, including the work on  structural graph parameters by
Bodlaender, Jansen, and
Kratsch~\cite{BodlaenderJansenKratsch2011,JansenKratsch2011a,JansenKratsch2011b},
which we have not investigated. It is also unknown whether
\textsc{Multi-tape NDTM Halting}$(k\log n)$ is in \WK[2].
Furthermore, it would be interesting to know some natural
parameterized problems which are \WK[2]-complete under a
standard parameter (e.g., $k$ rather than $k\log n$). On the
more structural side, we have noted several connections between
our hierarchy and previous hierarchies. It would be interesting
if these could be made stronger. In particular, we would like
to know if there are (classical or parameterized) complexity
theoretical implications of polynomial Turing kernelizations
for \WK[1].

